Lumbar Bone Mineral Density Estimation from Chest X-ray Images: Anatomy-aware Attentive Multi-ROI Modeling

Osteoporosis is a common chronic metabolic bone disease often under-diagnosed and under-treated due to the limited access to bone mineral density (BMD) examinations, e.g. via Dual-energy X-ray Absorptiometry (DXA). This paper proposes a method to predict BMD from Chest X-ray (CXR), one of the most commonly accessible and low-cost medical imaging examinations. Our method first automatically detects Regions of Interest (ROIs) of local CXR bone structures. Then a multi-ROI deep model with transformer encoder is developed to exploit both local and global information in the chest X-ray image for accurate BMD estimation. Our method is evaluated on 13719 CXR patient cases with ground truth BMD measured by the gold standard DXA. The model predicted BMD has a strong correlation with the ground truth (Pearson correlation coefficient 0.894 on lumbar 1). When applied in osteoporosis screening, it achieves a high classification performance (average AUC of 0.968). As the first effort of using CXR scans to predict the BMD, the proposed algorithm holds strong potential for early osteoporosis screening and public health promotion.

==> tables/ablationEnsemble.tex <==
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Ensemble} & \multicolumn{2}{c|}{L1}         & \multicolumn{2}{c|}{L2}         & \multicolumn{2}{c|}{L3}         & \multicolumn{2}{c|}{L4}         & \multicolumn{2}{c|}{Average}    \\ \cline{2-11} 
%                           & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            \\ \hline\hline
% Ensm\_roi             & 0.879          & 0.935          & 0.876          & 0.946          & 0.850          & 0.929          & 0.812          & 0.894          & 0.854          & 0.926          \\ \hline
% Ensm\_all             & \textbf{0.881} & \textbf{0.938} & \textbf{0.880} & \textbf{0.949} & \textbf{0.851} & \textbf{0.933} & \textbf{0.816} & \textbf{0.903} & \textbf{0.857} & \textbf{0.931} \\ \hline
% \end{tabular}

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Ensemble} & \multicolumn{2}{c|}{L1}         & \multicolumn{2}{c|}{L2}         & \multicolumn{2}{c|}{L3}         & \multicolumn{2}{c|}{L4}         & \multicolumn{2}{c|}{Average}    \\ \cline{2-11} 
%                           & R-value        & RMSE            & R-value        & RMSE            & R-value        & RMSE            & R-value        & RMSE            & R-value        & RMSE            \\ \hline\hline
% Base            & 0.879          & 0.11          & 0.876          & 0.134          & 0.850          & 0.129          & 0.812          & 0.139          & 0.854          & 0.128          \\ \hline
% All             & \textbf{0.888} & \textbf{0.102} & \textbf{0.886} & \textbf{0.108} & \textbf{0.869} & \textbf{0.125} & \textbf{0.815} & 0.141 & \textbf{0.864} & \textbf{0.119} \\ \hline
% \end{tabular}


\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Ensemble} & \multicolumn{2}{c|}{L1}         & \multicolumn{2}{c|}{L2}         & \multicolumn{2}{c|}{L3}         & \multicolumn{2}{c|}{L4}         & \multicolumn{2}{c|}{Average}    \\ \cline{2-11} 
                          & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            \\ \hline\hline
Bases            & 0.879          & 0.935          & 0.876          & 0.946          & 0.850          & 0.929          & 0.812          & 0.894          & 0.854          & 0.926          \\ \hline
All             & \textbf{0.888} & \textbf{0.947} & \textbf{0.886} & \textbf{0.954} & \textbf{0.869} & \textbf{0.939} & \textbf{0.815} & \textbf{0.907} & \textbf{0.864} & \textbf{0.937} \\ \hline
\end{tabular}


% Ensemble of 5 ROI models:
% 0.879	0.877	0.854	0.811	0.855
% 0.11	0.134	0.129	0.139	0.128
% roc_auc:  {0: 0.935, 1: 0.946, 2: 0.929, 3: 0.894, 'avg': 0.926}

% Ensemble of all 6 models: 
% 0.888	0.886	0.869	0.815	0.864
% 0.102	0.108	0.125	0.141	0.119
% roc_auc:  {0: 0.947, 1: 0.954, 2: 0.939, 3: 0.907, 'avg': 0.937}


==> tables/ablation_sexage.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Patch} & \multicolumn{3}{c|}{L1}                           & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           & \multicolumn{3}{c|}{Avg}                          \\\cline{2-16} 
                       & R-Val        & RMSE           & AUC            & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & R-val        & RMSE           & AUC            \\\hline
All & 0.888  & 0.067 & 0.963 & 0.889  & 0.076 & 0.964 & 0.878  & 0.082 & 0.971 & 0.840  & 0.095 & 0.966 & 0.874  & 0.080  & 0.966 \\\hline
M40-50                      & 0.845  & 0.067 & 0.980 & 0.848  & 0.076 & 0.992 & 0.842  & 0.080 & 0.990 & 0.822  & 0.085 & 0.947 & 0.839  & 0.077  & 0.977 \\\hline
M50-60                      & 0.866  & 0.065 & 0.940 & 0.857  & 0.076 & 0.926 & 0.844  & 0.080 & 0.955 & 0.801  & 0.094 & 0.955 & 0.842  & 0.079  & 0.944 \\\hline
M60-70                      & 0.820  & 0.077 & 0.978 & 0.795  & 0.089 & 0.972 & 0.779  & 0.101 & 0.922 & 0.726  & 0.116 & 0.994 & 0.780  & 0.095  & 0.966 \\\hline
M70-90                      & 0.884  & 0.077 & 0.980 & 0.876  & 0.091 & 0.977 & 0.851  & 0.103 & 0.966 & 0.833  & 0.115 & 0.953 & 0.861  & 0.096  & 0.969 \\\hline
F40-50                      & 0.871  & 0.060 & 0.970 & 0.866  & 0.068 & 0.983 & 0.870  & 0.070 & 0.997 & 0.838  & 0.083 & 0.978 & 0.861  & 0.070  & 0.982 \\\hline
F50-60                      & 0.897  & 0.060 & 0.946 & 0.904  & 0.064 & 0.948 & 0.896  & 0.071 & 0.958 & 0.864  & 0.085 & 0.943 & 0.890  & 0.070  & 0.949 \\\hline
F60-70                      & 0.882  & 0.065 & 0.931 & 0.889  & 0.074 & 0.932 & 0.886  & 0.080 & 0.936 & 0.820  & 0.104 & 0.926 & 0.869  & 0.081  & 0.931 \\\hline
F70-90                      & 0.798  & 0.093 & 0.873 & 0.777  & 0.098 & 0.878 & 0.805  & 0.106 & 0.883 & 0.777  & 0.120 & 0.912 & 0.789  & 0.104  & 0.886
       
  \\\hline
\end{tabular}


% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{}{}{Data} & \multicolumn{3}{c|}{L1}                              & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}
%             & \multicolumn{1}{c|}{train}& \multicolumn{1}{c|}{test}
% \\ \cline{2-13} 
% Range & R-value & RMSE   & AUC    & R-value & RMSE   & AUC    & R-value & RMSE   & AUC    & R-value & RMSE   & AUC    & \multirow{}{}{\#} & \multirow{}{}{\#} \\ \hline 
% All  & 0.8885  & 0.0669  & 0.9626 & 0.8892  & 0.0757 & 0.9644 & 0.8776  & 0.0815 & 0.9713 & 0.8399   & 0.0954 & 0.9658 & 11024                      & 2695                      \\ \hline  \hline
% M40-50                       & 0.8454  & 0.0673 & 0.9802 & 0.848   & 0.0755 & 0.9915 & 0.842   & 0.0796 & 0.9895 & 0.822   & 0.0849 & 0.9473 & 1605                       & 372                       \\ \hline
% M50-60                       & 0.8663  & 0.0651 & 0.9396 & 0.8567  & 0.0759 & 0.9259 & 0.8437  & 0.0799 & 0.955  & 0.8012  & 0.0943 & 0.9545 & 2095                       & 499                       \\ \hline
% M60-70                       & 0.8196  & 0.0766 & 0.9776 & 0.7953  & 0.089  & 0.9719 & 0.7792  & 0.1006 & 0.9218 & 0.7261  & 0.1156 & 0.9943 & 1258                       & 292                       \\ \hline
% M70-90                       & 0.8836  & 0.0768 & 0.9796 & 0.876   & 0.0912 & 0.9765 & 0.8509  & 0.1027 & 0.966  & 0.8328  & 0.1149 & 0.9532 & 468                        & 123                       \\ \hline
% F40-50                       & 0.8705  & 0.0599 & 0.9703 & 0.8657  & 0.0678 & 0.9833 & 0.8695  & 0.0699 & 0.9967 & 0.8378  & 0.0829 & 0.9784 & 1589                       & 435                       \\ \hline
% F50-60                       & 0.8966  & 0.0596 & 0.9457 & 0.904   & 0.0638 & 0.948  & 0.8956  & 0.0713 & 0.9581 & 0.8637  & 0.0848 & 0.9432 & 2279                       & 564                       \\ \hline
% F60-70                       & 0.8823  & 0.0646 & 0.931  & 0.8891  & 0.0743 & 0.9318 & 0.8859  & 0.0797 & 0.9356 & 0.8199  & 0.1044 & 0.9259 & 1205                       & 277                       \\ \hline
% F70-90                       & 0.7981  & 0.0926 & 0.8731 & 0.7766  & 0.0981 & 0.8777 & 0.8051  & 0.1058 & 0.8831 & 0.7769  & 0.1202 & 0.9119 & 525                        & 133                      

%       \\ \hline
% \end{tabular}


==> tables/baseline_backbones.tex <==

\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Backbone} & \multicolumn{3}{c|}{L1}                           & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           & \multicolumn{3}{c|}{Avg}                          \\\cline{2-16} 
                       & R-Val        & RMSE           & AUC            & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & R-val        & RMSE           & AUC            \\\hline
VGG13                     & 0.864          & 0.075          & 0.954          & 0.865          & 0.084          & 0.956          & 0.862          & 0.088          & 0.965          & \textbf{0.828} & 0.099          & 0.957          & 0.855 & 0.086          & 0.958          \\\hline
VGG16                     & \textbf{0.866} & \textbf{0.074} & \textbf{0.956} & \textbf{0.870} & 0.083          & 0.959          & \textbf{0.863} & \textbf{0.086} & \textbf{0.966} & 0.822          & 0.103          & 0.959          & \textbf{0.855} & 0.086          & \textbf{0.960} \\\hline
VGG19                     & 0.863          & 0.075          & 0.955          & \textbf{0.870} & \textbf{0.082} & 0.958          & 0.861          & 0.087          & 0.961          & 0.824          & \textbf{0.098} & \textbf{0.960} & 0.855 & \textbf{0.085} & 0.958          \\\hline
ResN18                    & 0.831          & 0.082          & 0.943          & 0.846          & 0.093          & 0.955          & 0.835          & 0.095          & 0.953          & 0.794          & 0.106          & 0.953          & 0.826          & 0.094          & 0.951          \\\hline
ResN34                    & 0.845          & 0.078          & 0.948          & 0.851          & 0.088          & 0.957          & 0.843          & 0.092          & \textbf{0.966} & 0.804          & 0.105          & 0.953          & 0.836          & 0.091          & 0.956          \\\hline
ResN50                    & 0.852          & 0.078          & 0.949          & 0.857          & 0.085          & \textbf{0.961} & 0.852          & 0.092          & 0.964          & 0.814          & 0.104          & 0.957          & 0.844          & 0.090          & 0.958          \\\hline
ResN101                   & 0.846          & 0.078          & 0.949          & 0.860          & 0.087          & 0.959          & 0.855          & 0.090          & 0.965          & 0.805          & 0.105          & 0.955          & 0.841          & 0.090          & 0.957         
  \\\hline
\end{tabular}



% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Baseline} & \multicolumn{3}{c|}{L1}                              & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           \\ \cline{2-13} 
%       & R-value   & RMSE   & AUC   & R-value & RMSE  & AUC & R-value   & RMSE  & AUC & R-value    & RMSE   & AUC \\ \hline\hline
% VGG13                              & 0.8638          & 0.0748          & 0.9541          & 0.8647          & 0.0835         & 0.9563          & 0.8616          & 0.0877          & 0.9651          & 0.8281          & 0.0994          & 0.9565          \\ \hline
% VGG16                              & \textbf{0.8661} & \textbf{0.0744} & \textbf{0.9557} & 0.8696          & 0.0825         & 0.9585          & \textbf{0.8625} & \textbf{0.0863} & 0.9655          & 0.8222          & 0.1025          & 0.9586          \\ \hline
% VGG19                              & 0.8632          & 0.0745          & 0.9547          & \textbf{0.8702} & \textbf{0.082} & 0.9581          & 0.8613          & 0.0869          & 0.9606          & \textbf{0.8289} & \textbf{0.0983} & \textbf{0.9596} \\ \hline
% Resnet18                           & 0.8306          & 0.0818          & 0.9434          & 0.8461          & 0.0927         & 0.9548          & 0.8349          & 0.0949          & 0.9531          & 0.7939          & 0.1062          & 0.9526          \\ \hline
% Resnet34                           & 0.8445          & 0.0783          & 0.9478          & 0.8507          & 0.0879         & 0.9573          & 0.8429          & 0.0921          & \textbf{0.9658} & 0.8044          & 0.1054          & 0.9529          \\ \hline
% Resnet50                           & 0.8519          & 0.0781          & 0.9487          & 0.8566          & 0.0853         & \textbf{0.9606} & 0.8522          & 0.092           & 0.9643          & 0.8136          & 0.1043          & 0.957           \\ \hline 
% Resnet101                          & 0.8461          & 0.0775          & 0.9493          & 0.8597          & 0.0873         & 0.9586          & 0.8551          & 0.09            & 0.9649          & 0.8049          & 0.1046          & 0.9554         

%       \\ \hline
% \end{tabular}


==> tables/data_analyze_RMSE.tex <==

\begin{tabular}{|c||c|c|c|c|}
\hline
RMSE & L1     & L2     & L3     & L4     \\\hline\hline
L1   & 0.000 & 0.101 & 0.177 & 0.192 \\\hline
L2   & 0.101 & 0.000 & 0.101 & 0.129 \\\hline
L3   & 0.177 & 0.101 & 0.000 & 0.079 \\\hline
L4   & 0.192 & 0.129 & 0.079 & 0.000 \\\hline
\end{tabular}


==> tables/data_analyze_Rvalue.tex <==

\begin{tabular}{|c||c|c|c|c|}
\hline
R-values & L1     & L2     & L3     & L4     \\ \hline\hline
L1       & 1.000 & 0.918 & 0.878 & 0.807 \\\hline
L2       & 0.918 & 1.000 & 0.931 & 0.836 \\\hline
L3       & 0.878 & 0.931 & 1.000 & 0.898 \\\hline
L4       & 0.807 & 0.836 & 0.898 & 1.000 \\\hline
\end{tabular}


==> tables/multiPatchDim.tex <==


\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Patch} & \multicolumn{3}{c|}{L1}                           & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           & \multicolumn{3}{c|}{Avg}                          \\\cline{2-16} 
                       & R-Val        & RMSE           & AUC            & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & R-val        & RMSE           & AUC            \\\hline
2 x 2                      & 0.861          & 0.075          & 0.954          & 0.868          & 0.082          & 0.962          & 0.858          & 0.088          & 0.965          & 0.821          & 0.100          & 0.960          & 0.852          & 0.086          & 0.960          \\\hline
3 x 3                     & 0.872 & 0.071 & 0.960 & 0.880 & 0.079 & \textbf{0.966} & 0.874 & 0.083 & 0.970 & 0.834          & 0.096          & 0.963          & 0.865 & 0.082 & 0.965 \\\hline
4 x 4                      & 0.867          & 0.073          & 0.956          & 0.876          & 0.080          & 0.964          & 0.867          & 0.085          & 0.966          & 0.836 & 0.096 & 0.966 & 0.861          & 0.083          & 0.963         
  \\\hline
\textbf{Ours}              & \textbf{0.889} & \textbf{0.067} & \textbf{0.963} & \textbf{0.889}              & \textbf{0.076}           & 0.964                   & \textbf{0.878}              & \textbf{0.082}           & \textbf{0.971}          & \textbf{0.840}              & \textbf{0.095}           & \textbf{0.966}          & \textbf{0.874} & \textbf{0.080} & \textbf{0.966} \\\hline


\end{tabular}







% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Multi-Patch} & \multicolumn{3}{c|}{L1}                              & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           \\ \cline{2-13} 
%       & R-value   & RMSE   & AUC   & R-value & RMSE  & AUC & R-value   & RMSE  & AUC & R-value    & RMSE   & AUC \\ \hline\hline
% 2 * 2                                                                        & 0.8606          & 0.0747          & 0.9538          & 0.8683          & 0.0823          & 0.962           & 0.8583          & 0.0877          & 0.9651          & 0.821           & 0.0998          & 0.9601          \\ \hline
% 3 * 3                                                                        & \textbf{0.8719} & \textbf{0.0707} & \textbf{0.9603} & \textbf{0.8803} & \textbf{0.0787} & \textbf{0.9658} & \textbf{0.8735} & \textbf{0.0825} & \textbf{0.9697} & 0.8344          & 0.0964          & 0.9628          \\ \hline
% 4 * 4                                                                        & 0.8666          & 0.0728          & 0.9564          & 0.8762          & 0.0797          & 0.9637          & 0.8668          & 0.0845          & 0.9659          & \textbf{0.8357} & \textbf{0.0959} & \textbf{0.9658}
%       \\ \hline
% \end{tabular}



==> tables/networkComparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Backbone} & \multicolumn{2}{c|}{L1}         & \multicolumn{2}{c|}{L2}         & \multicolumn{2}{c|}{L3}         & \multicolumn{2}{c|}{L4}         & \multicolumn{2}{c|}{Average}    \\ \cline{2-11} 
                          & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            \\ \hline\hline

Resnet18                  & 0.759          & 0.875          & 0.799          & 0.863          & 0.774          & 0.852          & 0.717          & 0.840          & 0.762          & 0.858          \\ \hline
Resnet34                  & 0.787          & 0.903          & 0.787          & 0.866          & 0.768          & 0.887          & 0.723          & 0.861          & 0.766          & 0.879          \\ \hline
Resnet50                  & 0.799          & 0.894          & 0.823          & 0.888          & 0.795          & 0.880          & 0.741          & 0.858          & 0.789          & 0.880          \\ \hline
Vgg11                     & 0.843          & 0.919          & 0.838          & \textbf{0.916} & \textbf{0.832} & 0.917          & 0.772          & 0.881          & 0.821          & 0.908          \\ \hline
Vgg16                     & \textbf{0.865} & \textbf{0.923} & \textbf{0.863} & 0.913          & 0.824          & \textbf{0.918} & \textbf{0.804} & \textbf{0.901} & \textbf{0.839} & \textbf{0.914} \\ \hline
\end{tabular}




